Data Exchange Markets via Utility Balancing

This paper explores the design of a balanced data-sharing marketplace for entities with heterogeneous datasets and machine learning models that they seek to refine using data from other agents. The goal of the marketplace is to encourage participation for data sharing in the presence of such heterogeneity. Our market design approach for data sharing focuses on interim utility balance, where participants contribute and receive equitable utility from refinement of their models. We present such a market model for which we study computational complexity, solution existence, and approximation algorithms for welfare maximization and core stability. We finally support our theoretical insights with simulations on a mean estimation task inspired by road traffic delay estimation.

==> extra.tex <==
\section{Warm-up: Separable Linear Case}

\kamesh{This case appears unmotivated. I think the fully separable case -- $u_i(S) = \sum_{j \in S} w_{ij}$, with either proportional or Shapley sharing is better motivated. I prefer writing the general case first and then talking about special cases.}

Consider the case in \cref{example:linear}
where $u_i(S)=\min(\abs{S}, n_i)$
for an integer $n_i$ and
the cost-sharing is $h_{ij}(S)=\min\left(1, \frac{n_i}{\abs{S}}\right)$.

\igov{We need a lemma that says that the optimal
solution here will involve setting $x_{iS}=1$
for some $S$ for every $i$.}

We solve this case via a min-cost circulation.
We create the following network: For every agent $i$,
create two nodes $i_{in},i_{out}$. There is an arc
$(i_{in},i_{out})$ of capacity $n_i$ and cost $-1$.
For directed edge $(j,i)\in E(G)$, we add an arc $(j_{out},i_{in})$
of cost 0 and capacity 1. We view the flow in this
arc as $h_{ij}(S)$. Observe that the balance 
constraint is satisfied 
because of conservation of flow and that minimizing the cost of the circulation maximizes the utility.

We argue now that an integer min-cost circulation
in this network will find a socially optimal solution.

\begin{lemma}
    Given any solution $\{S_i\}_{i}$, there is another
    solution $\{T_i\}_{i} $ such that
    \begin{itemize}
        \item $\forall~i,\abs{T_i}\leq n_i$.
        \item $\forall~i, u_i(T_i)\geq 
         u_i(S_i)$.
    \end{itemize}
\end{lemma}
\begin{proof}
    We construct the same network as before. We now
    add an upper and lower bound of $u_i(S_i)$
    on each $(i_{in},i_{out})$ arc.
    Since the $\{S_i\}_i $ defined a flow, there is a feasible flow for this 
    network.
    But since all upper and lower bounds are integers,
    there is an integral circulation on this network.
\end{proof}



\begin{theorem}
    There is a polynomial-time algorithm to find a social welfare optimum solution. This is also guaranteed to be core stable.
\end{theorem}
\begin{proof}
We find a min-cost circulation. Observing that any circulation defines a feasible solution and vice versa, the min-cost circulation
finds the social welfare maximizing solution.

Suppose the solution found is not core-stable.
Then there is a subset of users who can modify their flow to increase their utilities. But then this set 
of users would correspond to an augmenting cycle in 
the circulation. Augmenting along this cycle would 
decrease the cost of the circulation.
\end{proof}



\begin{theorem}
    If the utilities are not symmetric, the gap 
    between the core-stable solution and the 
    socially-optimal solution is $\Omega(n)$.
\end{theorem}
\begin{proof}
\begin{figure}[h]
    \centering
    \includegraphics{img/lowerbounds-n.pdf}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

Set $u_{v_1}(S)=1+\epsilon$ if $v_n\in S$
and $u_{v_1}(\{v_2\})=1$.
Set $h_{v_1v_n}(S)=1+\epsilon$ if $v_n\in S$. Set
$u_{v_n}(\{v_1\})=1+\epsilon$.
For all other users, set $u_{v_i}(\{v_{i+1} \})=1$.

The solution that maximizes social welfare
sets $x_{v_1 \{v_n\}}=\frac{1}{1+\epsilon}$
and $x_{v_i\{v_{i+1} \} }=1 $
for all $i\neq 1,n+1$.
This gives a social welfare of $n$.

However, this solution is not core-stable.
The solution $x_{v_1\{v_n\}}=x_{v_n\{v_1\}}=1+\epsilon$ is core-stable
but only achieves a social welfare of $2+2\epsilon$. This gives a gap
of $\Omega(n)$.

\end{proof}

\begin{proof}
In \cref{fig:enter-label}, agent $i$ can receive data from $j$ iff there is a directed edge $(i,j)$. We set $u_i(S) = \sqrt{|S|}$ for every agent $i$ except $p,v$. Since we use proportional sharing, we set $h_{ij}(S)=\frac{u_i(S)}{\abs{S}} = \frac{1}{\sqrt{|S|}}$. We set $u_p(\{u\})=\sqrt{k}$ and $u_v(\{p\})=\sqrt{k}$. Note that though these utilities are not bounded above by one, we can make them so by scaling them down by the largest possible utility; this will not change the proof.

We first lower bound the optimal welfare. Consider the cycle $(z_1,u,p_1,v,z_{n},\ldots,z_1)$. Each user can send its data only to the next member in the cycle, and receive data only from the previous member in the cycle. One maximal feasible solution along this cycle yields utility $1$ for each agent, and we get a social welfare at least $n+2$. 
\begin{figure}[htbp]
    \centering   
    \includegraphics{img/lowerbounds-sqrtn-modified.pdf}    
    \caption{Instance for showing \cref{thm:core-neg}. }
    \label{fig:enter-label}
\end{figure}
Now, consider any core-stable solution. We will upper bound its welfare. In this solution, for agent $u$, let $\beta = \sum_{S | z_1 \in S} x_{uS}$, and let $A = \E\left[ \frac{1}{\sqrt{|S|}} \ | z_1 \in S \right]$. Denote the utility of any agent $w$ by $U(w)$. Then $U(z_1) = \beta \cdot A$, and by balance, 
\begin{equation}
    \label{eq:welf1}
    \sum_{i =1}^n U(z_i) = n \cdot \beta \cdot A \le n \cdot A.
\end{equation}
Note that $U(u), U(p), U(v) \le \sqrt{k}$, and by balance $\sum_{i=1}^{k-1} U(q_i) \le \sqrt{k}$. Therefore, 
\begin{equation}
    \label{eq:welf2} 
    U(u) + U(v) + U(p) + \sum_{i=1}^{k-1} U(q_i) \le 4 \sqrt{k}.
\end{equation}
Further note that by balance, $U(u) = U(p) = U(v)$. We will now upper bound $A$ and choose $k$ appropriately. 

Let $\ell = k-1$. Consider agent $u$ again. In the event $z_1 \notin S$, the maximum utility achievable is $\sqrt{\ell}$. Therefore,
\begin{equation}
\label{eq:ub1}
U(u) \le (1-\beta) \cdot \sqrt{\ell} + \beta \cdot \E[\sqrt{|S|} \ | z_1 \in S].
\end{equation}

\kamesh{This step is only correct if we restrict to the space of solutions satisfying the Pigou-Dalton Principle.}
If $U(p) = U(v) = U(u) < \sqrt{\ell}$, then all of $\{u,p,v, \cdot q_1, q_2, \ldots q_{\ell}\}$ can deviate and use the maximum welfare solution on only these agents. This solution yields maximum possible utility to all the agents; in particular, agent $u$ gets utility $\sqrt{\ell} > U(u)$. Since the current solution is core-stable, this deviation is disallowed, and we must have $U(u) \ge \sqrt{\ell}$. Plugging this into \cref{eq:ub1}, we have
$$ \E[\sqrt{|S|} \ | z_1 \in S] \ge \sqrt{\ell}. $$
where we have $|S| \le \ell + 1$. Let $\gamma = \Pr[|S| \ge \ell/4]$.  Then the above implies
$$ \gamma \cdot \sqrt{\ell+1} + (1-\gamma) \cdot \frac{\sqrt{\ell}}{2} \ge \sqrt{\ell}.$$
Simplifying, we obtain
$$ \gamma \ge \frac{\sqrt{\ell}}{2 \sqrt{\ell+1} - \sqrt{\ell}}.$$
Note now that
\begin{align*}
    A  & =  \E\left[\frac{1}{\sqrt{|S|}} \ | z_1 \in S\right]  \le (1-\gamma)\cdot 1 + \gamma \cdot \frac{2}{\sqrt{\ell}}  \\
      & \le 2 \frac{\sqrt{\ell+1} - \sqrt{\ell}}{2 \sqrt{\ell+1} - \sqrt{\ell}} + \frac{2}{\sqrt{\ell}} \\
      & \le \frac{1}{\sqrt{\ell}} \cdot \frac{1}{2 \sqrt{\ell+1} - \sqrt{\ell}} + \frac{2}{\sqrt{\ell}} \le \frac{3}{\sqrt{\ell}} \le \frac{4}{\sqrt{k}}.
\end{align*}

Combining this with \cref{eq:welf1,eq:welf2}, the total utility of the solution is 
$$  U(u) + U(v) + U(p) + \sum_{i=1}^{k-1} U(q_i) + \sum_{i =1}^n U(z_i)\le   4 \sqrt{k} + n \cdot A \le 4 \left(\sqrt{k} + \frac{n}{\sqrt{k}}\right) \le 8 \sqrt{n},$$
where we have set $k = n$. Therefore the gap between the welfare of the core solution and the social welfare maximizing solution is $\Omega(\sqrt{n})$.


%%%
%%% This case seems too specific
\iffalse
\subsection{Case 2}
Like before, we have weights $w_{ij}$.
The utility is now defined by \[
u_i(S)=\max_{j\in S} w_{ij}
\]
Suppose $S=\{j_1,j_2,\ldots\}$, such that
$w_{ij_1}<w_{ij_2}<\ldots$.
Then $h_{ij_k}(S)=w_{ij_{k}}-w_{ij_{k-1}}$
where $w_{ij_0}:=0$.

\begin{theorem}
    The dual oracle is solvable in polynomial time.
\end{theorem}
\begin{proof}
    Like before, we can ignore
    $j$ such that $Q_{ij}<0$.

    Among the remaining $j$s, we sort them in decreasing order of $w_{ij}$. Then $S$ will be determined by the largest monotonically increasing set of 
    $Q_{ij}$s. To see this,
    suppose that we had $j_1,j_2\in S$ with $w_{ij_1}>w_{ij_2}$ and
    no other agents have $w_{ij}\in (w_{ij_2},w_{ij_1})$.
    If $Q_{ij_1}>Q_{ij_2}$,
    then it is strictly better
    to remove $j_1$ from $S$ because
    it increases the total utility.
\end{proof}
\fi 





\begin{theorem}
\label{thm:core-neg}
    For
    both
    the proportional sharing rule,
    and the Shapley value, there are instances where the gap in social welfare between any core-stable solution and the welfare-optimal solution is %$\Omega(\sqrt{n})$.
    $\Omega(n)$.
\end{theorem}
\begin{proof}
\begin{figure}[htbp]
    \centering   
    %\includegraphics{img/lowerbounds-sqrtn.pdf}    
    \includegraphics{img/lowerbounds-n.pdf}
    \caption{Instance for showing Theorem~\ref{thm:core-neg}. }
    \label{fig:enter-label}
\end{figure}



In Figure~\ref{fig:enter-label}, agent $i$ can receive data from $j$ iff there is a directed edge $(i,j)$.  We set $u_i(S) = |S|^c$ for some $c\leq 1$ every agent $i$. Since we use proportional sharing, we set $h_{ij}(S)=\frac{u_i(S)}{\abs{S}} = |S|^{c-1}$.
    
Consider the cycle $(z_1,u,p_1,v,z_{n},\ldots,z_1)$. Each user can send its data only to the next member in the cycle, and receive data only from the previous member in the cycle. The maximal feasible solution along this cycle yields utility $1$ for each agent, and we get a social welfare of $n+2$. 

Now, we show that any core-stable  solution has a large gap in utility compared to the previous solution. 
Consider the agents assigned to $u$.

\kamesh{Show that any core-stable solution sends small-flow.}


\begin{alignat*}{2}
    x_{uS}&=1  &&\text{ for }S=\{z_1,q_1,\ldots,q_{k-1} \}\\
    x_{vS}&=1 &&\text{ for }S=\{p_1,\ldots,p_k\}\\
    x_{z_i\{z_{i+1} \} }&=k^{\alpha-1} &&\text{ for } i\in[n-1] \\
    x_{p_i\{u\} }&=k^{\alpha-1} && \text{ for } i\in [k] \\
    x_{q_i\{v\} }&=k^{\alpha-1} && \text{ for } i\in [k-1] \\
    x_{z_n\{v\} }&=k^{\alpha-1}.
\end{alignat*}

Observe that the balance condition is satisfied.
For all users $i$, we can also set $x_{i\phi}$
appropriately so that \cref{eqn:probability-sum-1}
is satisfied.
Since $u,v$ receives the maximum possible utility it can, they have no incentive to deviate. Since there is no
cycle in the graph once $u,v$ are removed,
no set of users can increase their utilities
by trading between them.
Thus, this solution is core-stable.

The social welfare is $2k^\alpha+(n+2k-1)k^{\alpha-1}$. Choosing $k=\sqrt{n}$
and in the limit of $\alpha\to 0$, the gap is
$\Omega(\sqrt{n})$.

\end{proof}





The utility function for agent $i$ is an arbitrary monotone submodular function $u_i(S)$;  it is shared among the elements $j\in S$ as: 
\[
h_{ij}(S) = u_i(S) \frac{s_{ij}}{\sum_{k \in S} s_{ik}}
\]
Let $V(S) = \sum_{j \in S} Q_{ij} s_{ij}$ and $D(S) = \sum_{j \in S} s_{ij}$. The oracle problem (\cref{eqn:oracle}) becomes
$$ \max_{S \subseteq X \setminus \{i\}} u_i(S) \cdot \frac{V(S)}{D(S)}.$$


up to a constant
multiplicative factor
and an additive factor
of $\epsilon$.
Suppose we guess the optimal values of 
$u_i(S),R(S)$ and $W(S)$ to be $R^*,W^*$.
By guessing in terms of powers of $(1+\epsilon)$, we can do this in time
\igov{Todo: To get the log factor, lower bound the values.}
\begin{enumerate}
    \item $O(\log n)$ to guess $U^*$.
    \item $O(T \log n)$ to guess
    $R^*$, where $T=(\frac{8n^2\log n}{\epsilon^2})$ is the number
    of iterations in \cref{alg:mwu_general}.
    \item $O(\log (\sum_j w_j))=O(\log n)$ to guess $W^*$.
\end{enumerate}
which gives an overall running time of
$O(T\log^3n)$.
Since $W^*\geq 1$ and
$U^*\leq 1$,
we can assume that
$R^*\geq \epsilon$.
Otherwise, the objective
function is smaller than
$\epsilon$, in which
case we can return $\phi$
as our solution which
is still within an additive $\epsilon$ of the objective.

Let $F_i$ be the multilinear
relaxation of $u_i$.
Then an approximation
to the oracle would be to
\begin{align*}
    \text{Maximize } F_i(x) &\text{  s.t }\\
    \sum_j r_j x_j &\geq  R^*\\
    \sum_j w_j x_j &\leq W^*
\end{align*}
Let $X^+=\{j\in X: r_j>0\}$ and
$X^-=\{j\in X: r_j<0\}$. Then we
further guess $R^+,R^-\geq 0$
so that $R^+-R^-=R^*$.
For this guess, we can further simplify
the above oracle as
\begin{align*}
    \text{Maximize } F_i(x) &\text{  s.t }\\
    \sum_{j\in X^+} r_j x_j &\geq R^+\\
    \sum_{j\in X^-} (-r_j) x_j &\leq  R^-\\
    \sum_j w_j x_j &\le W^*
\end{align*}
This guess requires a further time
of $O(T\log n)$, since guessing $R^+$ immediately implies the guess for $R^-$.
We now have a submodular maximization
problem with two `packing' constraints
and one `covering' constraint.
This can be solved to a $(1-\frac{1}{e}-\epsilon)$
approximation
in time $n^{\mathrm{poly}(\frac{1}{\epsilon})}$ time
\cite{mizrachi2018tight}
such that the covering constraint
is violated by a factor of $(1-\epsilon)$.
\igov{Get the exact running time, including the dependency
on the numbers. Is it pseudo-polynomial time? If so, we will incur a cost of $R^*+W^*$.}


======

%We first consider the simplest case where the agents are all interested in one distribution. We have a set of $n$ users represented by integers $[n]$. User $i$  has $z^{(i)}$ samples of the distribution. An agent's objective is to decrease  the variance of their sample mean i.e. $\frac{\sigma^2}{z}$ where $z$ is the number of samples from the distribution that they have and $\sigma$ is the variance of the distribution. For a set of users $S\subseteq [n]$, let $z(S):=\sum_{i\in S}z^{(i)}$. Since agent $i$ starts with $z^{(i)}$ samples, the initial variance of her sample mean is $\frac{\sigma^2}{z^{(i)}}$. We represent her utility function as the decrease in variance.

%Thus,
%\begin{equation}\label{eqn:utility-variance}
%    u_i(S) = \frac{\sigma^2}{z^{(i)}}-\frac{\sigma^2}{z^{(i)}+z(S)}.
%\end{equation}
%Observe that $u_i(S)$ is a  concave function in terms of $z(S)$ and therefore, is submodular in terms of $S$. We do the cost-sharing according to the Shapley value.  Recall that the Shapley value is defined  in the following way. For a permutation $P$ of $[n]$, let $S_j^{P}$ be the set of users preceding $j$ in $P$.
%Then
%\[
%h_{ij}(S) = \mathop{\mathbb{E}}_{P\in \mathcal{P}_i}\left[ u_i(S_j^{P}\cup \{P\})-u_i(S_j^P) \right]
%\]
where $\mathcal{P}_i$ is the set of all
permutations of $[n]\setminus\{i\}$.
However,
since the Shapley value is computationally
expensive to compute, we estimate
it by sampling several random permutations
and computing the expectation over those
permutations.



This extends the utility function
in \cref{eqn:utility-variance}
in a natural way.
Note that the utility function
remains submodular since it 
is a sum of submodular functions.
We use synthetic data
for the samples, but
use a random subset of
Manhattan's streets
as our road network.

We run experiments on the task of mean estimation. The agents have several samples from a distribution, and their objective is to reduce the variance of their sample mean.

Our main conclusion
is that,
analogous to the Kidney exchange
problem,
the utility can be 
significantly improved by 
including cycles of length
more than two.
We also show that our algorithm
is robust to correlations (see Appendix~\cref{appendix}).

\iffalse
\subsection{Spatial Coverage}

There are some datasets with spatial features. For example, \url{file:///Users/sungjin/Downloads/Monitoring_the_Spread_of_Swine_Enteric_Coronavirus.pdf}
use three data sources to collect data on enteric coronavirus records in the United States. Maybe we can consider a simple coverage function with weights on states proportional to their population?

Satellite coverage data seems good, but it's hard to define mapping to locations. 
\fi 
